A Frobenius Algebraic Analysis for Parasitic Gaps

The interpretation of parasitic gaps is an ostensible case of non-linearity in natural language composition. Existing categorial analyses, both in the typelogical and in the combinatory traditions, rely on explicit forms of syntactic copying. We identify two types of parasitic gapping where the duplication of semantic content can be confined to the lexicon. Parasitic gaps in adjuncts are analysed as forms of generalized coordination with a polymorphic type schema for the head of the adjunct phrase. For parasitic gaps affecting arguments of the same predicate, the polymorphism is associated with the lexical item that introduces the primary gap. Our analysis is formulated in terms of Lambek calculus extended with structural control modalities. A compositional translation relates syntactic types and derivations to the interpreting compact closed category of finite dimensional vector spaces and linear maps with Frobenius algebras over it. When interpreted over the necessary semantic spaces, the Frobenius algebras provide the tools to model the proposed instances of lexical polymorphism.

==> Figures/coarg.tex <==
\begin{sidewaysfigure}
\[\resizebox{\textwidth}{!}{$\addtolength{\inferLineSkip}{2pt}
%\deduce{\textcolor{red}{\lambda z_{6}.((\textsc{sec\_{}breach} \  z_{6}) \wedge ((\textsc{made} \  z_{6}) \  \textsc{public}) \  (\textsc{a} \  ((\textsc{in} \  \textsc{NYT}) \  ((\textsc{about} \  z_{6}) \  \textsc{report}))))}}{\deduce{$\rule{0pt}{2em}$}{
   \infer[\textit{ev}^{\bs}]{\mbox{sec\_{}breach}\otimes_{}(\mbox{that}\otimes_{}((\mbox{a}\otimes_{}((\mbox{report}\otimes_{}\mbox{about})\otimes_{}(\mbox{in}\otimes_{}\mbox{NYT})))\otimes_{}(\mbox{made}\otimes_{}\mbox{public}))) \longrightarrow n}{
      \infer[\ell]{n}{\mbox{sec\_{}breach}}
   & 
      \infer[\textit{ev}^{/}]{\mbox{that}\otimes_{}((\mbox{a}\otimes_{}((\mbox{report}\otimes_{}\mbox{about})\otimes_{}(\mbox{in}\otimes_{}\mbox{NYT})))\otimes_{}(\mbox{made}\otimes_{}\mbox{public})) \longrightarrow n \bs_{}n}{
         \infer[\ell]{\mathit{relpro}}{\mbox{that}} %(n \bs_{}n) /_{}((np /_{}\diamondsuit_{}\Box_{}np) \otimes_{}((np \bs_{}s) /_{}\diamondsuit_{}\Box_{}np))
      & 
         \infer[\textsf{Mon}_{\otimes}]{(\mbox{a}\otimes_{}((\mbox{report}\otimes_{}\mbox{about})\otimes_{}(\mbox{in}\otimes_{}\mbox{NYT})))\otimes_{}(\mbox{made}\otimes_{}\mbox{public}) \longrightarrow (np /_{}\diamondsuit_{}\Box_{}np) \otimes_{}((np \bs_{}s) /_{}\diamondsuit_{}\Box_{}np)}{
            \infer[\textsf{Res}_{/}]{\mbox{a}\otimes_{}((\mbox{report}\otimes_{}\mbox{about})\otimes_{}(\mbox{in}\otimes_{}\mbox{NYT})) \longrightarrow np /_{}\diamondsuit_{}\Box_{}np}{
               \infer[\alpha_{\diamond}]{(\mbox{a}\otimes_{}((\mbox{report}\otimes_{}\mbox{about})\otimes_{}(\mbox{in}\otimes_{}\mbox{NYT})))\otimes_{}\diamondsuit^{}\Box_{}np \longrightarrow np}{
                  \infer[\sigma_{\diamond}]{\mbox{a}\otimes_{}(((\mbox{report}\otimes_{}\mbox{about})\otimes_{}(\mbox{in}\otimes_{}\mbox{NYT}))\otimes_{}\diamondsuit^{}\Box_{}np) \longrightarrow np}{
                     \infer[\alpha_{\diamond}]{\mbox{a}\otimes_{}(((\mbox{report}\otimes_{}\mbox{about})\otimes_{}\diamondsuit^{}\Box_{}np)\otimes_{}(\mbox{in}\otimes_{}\mbox{NYT})) \longrightarrow np}{
                        \infer[\textit{ev}^{/}]{\mbox{a}\otimes_{}((\mbox{report}\otimes_{}(\mbox{about}\otimes_{}\diamondsuit^{}\Box_{}np))\otimes_{}(\mbox{in}\otimes_{}\mbox{NYT})) \longrightarrow np}{
                           \infer[\ell]{np /_{}n}{\mbox{a}}
                        & 
                           \infer[\textit{ev}^{\bs}]{(\mbox{report}\otimes_{}(\mbox{about}\otimes_{}\diamondsuit^{}\Box_{}np))\otimes_{}(\mbox{in}\otimes_{}\mbox{NYT}) \longrightarrow n}{
                              \infer[\textit{ev}^{\bs}]{\mbox{report}\otimes_{}(\mbox{about}\otimes_{}\diamondsuit^{}\Box_{}np) \longrightarrow n}{
                                 \infer[\ell]{n}{\mbox{report}}
                              & 
                                 \infer[\textit{ev}^{/}]{\mbox{about}\otimes_{}\diamondsuit^{}\Box_{}np \longrightarrow n \bs_{}n}{
                                    \infer[\ell]{(n \bs_{}n) /_{}np}{\mbox{about}}
                                 & 
                                    \diamondsuit^{}\Box_{}np \longrightarrow np
                                 }
                              }
                           & 
                              \infer[\textit{ev}^{/}]{\mbox{in}\otimes_{}\mbox{NYT} \longrightarrow n \bs_{}n}{
                                 \infer[\ell]{(n \bs_{}n) /_{}np}{\mbox{in}}
                              & 
                                 \infer[\ell]{np}{\mbox{NYT}}
                              }
                           }
                        }
                     }
                  }
               }
            }
         & 
            \infer[\textsf{Res}_{/}]{\mbox{made}\otimes_{}\mbox{public} \longrightarrow (np \bs_{}s) /_{}\diamondsuit_{}\Box_{}np}{
               \infer[\sigma_{\diamond}]{(\mbox{made}\otimes_{}\mbox{public})\otimes_{}\diamondsuit^{}\Box_{}np \longrightarrow np \bs_{}s}{
                  \infer[\textit{ev}^{/}]{(\mbox{made}\otimes_{}\diamondsuit^{}\Box_{}np)\otimes_{}\mbox{public} \longrightarrow np \bs_{}s}{
                     \infer[\textit{ev}^{/}]{\mbox{made}\otimes_{}\diamondsuit^{}\Box_{}np \longrightarrow (np \bs_{}s) /_{}ap}{
                        \infer[\ell]{((np \bs_{}s) /_{}ap) /_{}np}{\mbox{made}}
                     & 
                        \diamondsuit^{}\Box_{}np \longrightarrow np
                     }
                  & 
                     \infer[\ell]{ap}{\mbox{public}}
                  }
               }
            }
         }
      }
   }%}}
$}\]
\caption{Co-argument parasitic gapping. \emph{relpro} abbreviates $(n \bs_{}n) /_{}((np /_{}\diamondsuit_{}\Box_{}np) \otimes_{}((np \bs_{}s) /_{}\diamondsuit_{}\Box_{}np))$.}
\label{coarg}
\end{sidewaysfigure}

==> Figures/parasitic_gap_derivation.tex <==
\[\resizebox{\textwidth}{!}{$\addtolength{\inferLineSkip}{2pt}
%\deduce{\textcolor{red}{\lambda z_{6}.((\textsc{paper} \  z_{6}) \wedge ((((\textsc{without{}} \  \textsc{reading}) \  \textsc{rejected}) \  z_{6}) \  \textsc{bob}))}}{\deduce{$\rule{0pt}{2em}$}{
   \infer[\textit{ev}^{\bs}]{\mbox{paper}\otimes_{}(\mbox{that}\otimes_{}(\mbox{bob}\otimes_{}(\mbox{rejected}\otimes_{}\rdia_{}(\mbox{without{}}\otimes_{}\mbox{reading})))) \longrightarrow n}{
      \infer[\ell]{n}{\mbox{paper}}
   & 
      \infer[\textit{ev}^{/}]{\mbox{that}\otimes_{}(\mbox{bob}\otimes_{}(\mbox{rejected}\otimes_{}\rdia_{}(\mbox{without{}}\otimes_{}\mbox{reading}))) \longrightarrow n \bs_{}n}{
         \infer[\ell]{(n \bs_{}n) /_{}(s /_{}\diamondsuit_{}\Box_{}np)}{\mbox{that}}
      & 
         \hspace{-3cm}\infer[\textsf{Res}_{/}]{\mbox{bob}\otimes_{}(\mbox{rejected}\otimes_{}\rdia_{}(\mbox{without{}}\otimes_{}\mbox{reading})) \longrightarrow s /_{}\diamondsuit_{}\Box_{}np}{
            \infer[\alpha_{\diamond}]{(\mbox{bob}\otimes_{}(\mbox{rejected}\otimes_{}\rdia_{}(\mbox{without{}}\otimes_{}\mbox{reading})))\otimes_{}\diamondsuit^{}\Box_{}np \longrightarrow s}{
               \infer[\textit{ev}^{\bs}]{\mbox{bob}\otimes_{}((\mbox{rejected}\otimes_{}\rdia_{}(\mbox{without{}}\otimes_{}\mbox{reading}))\otimes_{}\diamondsuit^{}\Box_{}np) \longrightarrow s}{
                  \infer[\ell]{np}{\mbox{bob}}
               & 
                  \hspace{-2cm}\infer[\textit{ev}^{/}]{(\mbox{rejected}\otimes_{}\rdia_{}(\mbox{without{}}\otimes_{}\mbox{reading}))\otimes_{}\diamondsuit^{}\Box_{}np \longrightarrow np \bs_{}s}{
                     \infer[\textit{ev}^{\bs}]{\mbox{rejected}\otimes_{}\rdia_{}(\mbox{without{}}\otimes_{}\mbox{reading}) \longrightarrow iv  /_{}np}{
                        \infer[\textsf{Res}_{/}]{\mbox{rejected} \longrightarrow iv  /_{}\diamondsuit_{}\Box_{}np}{
                           \infer[\textit{ev}^{/}]{\mbox{rejected}\otimes_{}\diamondsuit^{}\Box_{}np \longrightarrow np \bs_{}s}{
                              \infer[\ell]{iv  /_{}np}{\mbox{rejected}}
                           & 
                              \diamondsuit^{}\Box_{}np \longrightarrow np
                           }
                        }
                     & 
                        \infer[\textsf{Res}_{\Box}]{\rdia_{}(\mbox{without{}}\otimes_{}\mbox{reading}) \longrightarrow (iv  /_{}\diamondsuit_{}\Box_{}np) \bs_{}(iv  /_{}np)}{
                           \infer[\textit{ev}^{/}]{\mbox{without{}}\otimes_{}\mbox{reading} \longrightarrow \rbox_{}((iv  /_{}\diamondsuit_{}\Box_{}np) \bs_{}(iv  /_{}np))}{
                              \infer[\ell]{\rbox_{}((iv  /_{}\diamondsuit_{}\Box_{}np) \bs_{}(iv  /_{}np)) /_{}(gp /_{}\diamondsuit_{}\Box_{}np)}{\mbox{without{}}}
                           & 
                              \infer[\textsf{Res}_{/}]{\mbox{reading} \longrightarrow gp /_{}\diamondsuit_{}\Box_{}np}{
                                 \infer[\textit{ev}^{/}]{\mbox{reading}\otimes_{}\diamondsuit^{}\Box_{}np \longrightarrow gp}{
                                    \infer[\ell]{gp /_{}np}{\mbox{reading}}
                                 & 
                                    \diamondsuit^{}\Box_{}np \longrightarrow np
                                 }
                              }
                           }
                        }
                     }
                  & 
                     \hspace{-2cm}\diamondsuit^{}\Box_{}np \longrightarrow np
                  }
               }
            }
         }
      }
   }%}}
$}\]

==> Figures/parasitic_gap_simple2_derivation.tex <==
{\small\begin{equation*}
%\deduce{\textcolor{red}{(((\textsc{without} \  (\textsc{closing} \  (\textsc{the} \  \textsc{window}))) \  \textsc{left}) \  \textsc{bob})}}{\deduce{$\rule{0pt}{2em}$}{
   \infer[\textit{ev}^{\bs}]{\mbox{bob}\otimes_{}(\mbox{left}\otimes_{}\rdia_{}(\mbox{without}\otimes_{}(\mbox{closing}\otimes_{}(\mbox{the}\otimes_{}\mbox{window})))) \longrightarrow s}{
      \infer[\ell]{np}{\mbox{bob}}
   & 
      \infer[\textit{ev}^{\bs}]{\mbox{left}\otimes_{}\rdia_{}(\mbox{without}\otimes_{}(\mbox{closing}\otimes_{}(\mbox{the}\otimes_{}\mbox{window}))) \longrightarrow np \bs_{}s}{
         \infer[\ell]{np \bs_{}s}{\mbox{left}}
      & 
         \infer[\textsf{Res}_{\Box}]{\rdia_{}(\mbox{without}\otimes_{}(\mbox{closing}\otimes_{}(\mbox{the}\otimes_{}\mbox{window}))) \longrightarrow (np \bs_{}s) \bs_{}(np \bs_{}s)}{
            \infer[\textit{ev}^{/}]{\mbox{without}\otimes_{}(\mbox{closing}\otimes_{}(\mbox{the}\otimes_{}\mbox{window})) \longrightarrow \rbox_{}((np \bs_{}s) \bs_{}(np \bs_{}s))}{
               \infer[\ell]{\rbox_{}((np \bs_{}s) \bs_{}(np \bs_{}s)) /_{}gp}{\mbox{without}}
            & 
               \infer[\textit{ev}^{/}]{\mbox{closing}\otimes_{}(\mbox{the}\otimes_{}\mbox{window}) \longrightarrow gp}{
                  \infer[\ell]{gp /_{}np}{\mbox{closing}}
               & 
                  \infer[\textit{ev}^{/}]{\mbox{the}\otimes_{}\mbox{window} \longrightarrow np}{
                     \infer[\ell]{np /_{}n}{\mbox{the}}
                  & 
                     \infer[\ell]{n}{\mbox{window}}
                  }
               }
            }
         }
      }
   }%}}
\end{equation*}
}

==> Sections/ASampleDerivations.tex <==
\section{Sample derivations}

\paragraph*{Non-peripheral extraction}
Derivation for (\ref{data2}a), \emph{papers that Bob rejected \textvisiblespace{} immediately}.
The $\fdia\gbox np$ gap hypothesis finds its landing site adjacent to \emph{rejected} thanks to controlled
associativity $\overline{\alpha}_\diamond$ and commutativity $\overline{\sigma}_\diamond$.

\newcommand{\fboxx}[1]{#1}
% \renewcommand{\Diamond}{\fdia}

\[\addtolength{\inferLineSkip}{2pt}
%\begin{preview}
\scalebox{.8}{$\infer[\triangleleft^{-1}]{ n_{} \otimes (((n_{} \bs n_{})/ (s_{}/  \Diamond  \Box np_{})) \otimes (np_{} \otimes (((np_{} \bs s_{})/ np_{}) \otimes ((np_{} \bs s_{}) \bs (np_{} \bs s_{})))))  \longrightarrow n_{}}{
 \infer[\triangleright^{-1}]{ ((n_{} \bs n_{})/ (s_{}/  \Diamond  \Box np_{})) \otimes (np_{} \otimes (((np_{} \bs s_{})/ np_{}) \otimes ((np_{} \bs s_{}) \bs (np_{} \bs s_{}))))  \longrightarrow  n_{} \bs n_{} }{
 \infer[\slash ]{\fboxx{ (n_{} \bs n_{})/ (s_{}/  \Diamond  \Box np_{}) } \longrightarrow  (n_{} \bs n_{})/ (np_{} \otimes (((np_{} \bs s_{})/ np_{}) \otimes ((np_{} \bs s_{}) \bs (np_{} \bs s_{})))) }{
 \infer[\bs ]{\fboxx{ n_{} \bs n_{} } \longrightarrow  n_{} \bs n_{} }{
 \infer{\fboxx{n_{}} \longrightarrow n_{}}{} &  \infer{\fboxx{n_{}} \longrightarrow n_{}}{}} &  
 \infer[\overline{\alpha}_\diamond]{\colorbox{gray!20}{$ np_{} \otimes (((np_{} \bs s_{})/ np_{}) \otimes ((np_{} \bs s_{}) \bs (np_{} \bs s_{})))  \vdash  s_{}/  \Diamond  \Box np_{} $}}{
 \infer[\triangleright^{-1}]{ (((np_{} \bs s_{})/ np_{}) \otimes ((np_{} \bs s_{}) \bs (np_{} \bs s_{}))) \otimes  \Diamond  \Box np_{}  \longrightarrow  np_{} \bs s_{} }{
 \infer[\overline{\sigma}_\diamond]{ ((np_{} \bs s_{})/ np_{}) \otimes ((np_{} \bs s_{}) \bs (np_{} \bs s_{}))  \vdash  (np_{} \bs s_{})/  \Diamond  \Box np_{} }{
 \infer[\triangleright]{ ((np_{} \bs s_{})/ np_{}) \otimes  \Diamond  \Box np_{}  \longrightarrow  (np_{} \bs s_{})/ ((np_{} \bs s_{}) \bs (np_{} \bs s_{})) }{
 \infer[\triangleleft^{-1}]{\colorbox{gray!20}{$(((np_{} \bs s_{})/ np_{}) \otimes  \Diamond  \Box np_{}) \otimes ((np_{} \bs s_{}) \bs (np_{} \bs s_{}))  \longrightarrow  np_{} \bs s_{} $}}{
 \infer[\bs ]{\fboxx{ (np_{} \bs s_{}) \bs (np_{} \bs s_{}) } \longrightarrow  (((np_{} \bs s_{})/ np_{}) \otimes  \Diamond  \Box np_{}) \bs (np_{} \bs s_{}) }{
 \infer[\triangleright^{-1}]{ ((np_{} \bs s_{})/ np_{}) \otimes  \Diamond  \Box np_{}  \longrightarrow  np_{} \bs s_{} }{
 \infer[\slash ]{\fboxx{ (np_{} \bs s_{})/ np_{} } \longrightarrow  (np_{} \bs s_{})/  \Diamond  \Box np_{} }{
 \infer[\bs ]{\fboxx{ np_{} \bs s_{} } \longrightarrow  np_{} \bs s_{} }{
 \infer{\fboxx{np_{}} \longrightarrow np_{}}{} &  \infer{\fboxx{s_{}} \longrightarrow s_{}}{}} &  \infer[\triangledown^{-1}]{ \Diamond  \Box np_{} \vdash np_{}}{ \infer[\Box ]{\fboxx{ \Box np_{}} \vdash  \Box np_{}}{ \infer{\fboxx{np_{}} \longrightarrow np_{}}{}}}}} &  \infer[\bs ]{\fboxx{ np_{} \bs s_{} } \longrightarrow  np_{} \bs s_{} }{
 \infer{\fboxx{np_{}} \longrightarrow np_{}}{} &  \infer{\fboxx{s_{}} \longrightarrow s_{}}{}}}}}}}}}}}
$}%\end{preview}
\]

\paragraph*{Parasitic gap}
We present the derivation of (\ref{data2}d) ``papers that reviewers rejected \textvisiblespace{} without reading \textvisiblespace{} carefully'' in two formats. 
Figure \ref{allrules} shows both the invertible
residuation rules and the non-invertible rules (monotonicity, controlled associativity/commutativity).
Figure \ref{noninvertiblerules} only has the noninvertible rules that are responsible for composing complex formulas out of their subformulas. Atomic formula occurrences are indexed to highlight the matchings at
the axiom leaves. These matching fully determine the tensor contractions in the target sCCC for semantics
as explained in the text.

\begin{sidewaysfigure}

\begin{center}
\scalebox{.7}{\addtolength{\inferLineSkip}{2pt}
\infer[\triangleleft^{-1}]{ n_{} \otimes (((n_{} \bs n_{})/ (s_{}/  \Diamond  \Box np_{})) \otimes (np_{} \otimes (((np_{} \bs s_{})/ np_{}) \otimes  \Diamond (( \Box (((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))/ (gp_{}/  \Diamond  \Box np_{})) \otimes ((gp_{}/ np_{}) \otimes (gp_{} \bs gp_{}))))))  \longrightarrow n_{}}{
 \infer[\triangleright^{-1}]{ ((n_{} \bs n_{})/ (s_{}/  \Diamond  \Box np_{})) \otimes (np_{} \otimes (((np_{} \bs s_{})/ np_{}) \otimes  \Diamond (( \Box (((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))/ (gp_{}/  \Diamond  \Box np_{})) \otimes ((gp_{}/ np_{}) \otimes (gp_{} \bs gp_{})))))  \longrightarrow  n_{} \bs n_{} }{
 \infer[\slash ]{\fboxx{ (n_{} \bs n_{})/ (s_{}/  \Diamond  \Box np_{}) } \longrightarrow  (n_{} \bs n_{})/ (np_{} \otimes (((np_{} \bs s_{})/ np_{}) \otimes  \Diamond (( \Box (((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))/ (gp_{}/  \Diamond  \Box np_{})) \otimes ((gp_{}/ np_{}) \otimes (gp_{} \bs gp_{}))))) }{
 \infer[\bs ]{\fboxx{ n_{} \bs n_{} } \longrightarrow  n_{} \bs n_{} }{
 \infer{\fboxx{n_{}} \longrightarrow n_{}}{} &  \infer{\fboxx{n_{}} \longrightarrow n_{}}{}} &  \infer[\overline{\alpha}_\diamond]{ np_{} \otimes (((np_{} \bs s_{})/ np_{}) \otimes  \Diamond (( \Box (((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))/ (gp_{}/  \Diamond  \Box np_{})) \otimes ((gp_{}/ np_{}) \otimes (gp_{} \bs gp_{}))))  \vdash  s_{}/  \Diamond  \Box np_{} }{
 \infer[\triangleright^{-1}]{ (((np_{} \bs s_{})/ np_{}) \otimes  \Diamond (( \Box (((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))/ (gp_{}/  \Diamond  \Box np_{})) \otimes ((gp_{}/ np_{}) \otimes (gp_{} \bs gp_{})))) \otimes  \Diamond  \Box np_{}  \longrightarrow  np_{} \bs s_{} }{
 \infer[\triangleleft^{-1}]{ ((np_{} \bs s_{})/ np_{}) \otimes  \Diamond (( \Box (((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))/ (gp_{}/  \Diamond  \Box np_{})) \otimes ((gp_{}/ np_{}) \otimes (gp_{} \bs gp_{})))  \longrightarrow  (np_{} \bs s_{})/  \Diamond  \Box np_{} }{
 \infer[\triangledown^{-1}]{ \Diamond (( \Box (((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))/ (gp_{}/  \Diamond  \Box np_{})) \otimes ((gp_{}/ np_{}) \otimes (gp_{} \bs gp_{}))) \vdash  ((np_{} \bs s_{})/ np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}) }{ \infer[\triangleright^{-1}]{ ( \Box (((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))/ (gp_{}/  \Diamond  \Box np_{})) \otimes ((gp_{}/ np_{}) \otimes (gp_{} \bs gp_{}))  \longrightarrow  \Box (((np_{} \bs s_{})/ np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))}{
 \infer[\slash ]{\fboxx{  \Box (((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))/ (gp_{}/  \Diamond  \Box np_{}) } \longrightarrow   \Box (((np_{} \bs s_{})/ np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))/ ((gp_{}/ np_{}) \otimes (gp_{} \bs gp_{})) }{
 \infer[\Box ]{\fboxx{ \Box (((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))} \vdash  \Box (((np_{} \bs s_{})/ np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}))}{ \infer[\bs ]{\fboxx{ ((np_{} \bs s_{})/  \Diamond  \Box np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}) } \longrightarrow  ((np_{} \bs s_{})/ np_{}) \bs ((np_{} \bs s_{})/  \Diamond  \Box np_{}) }{
 \infer[\slash ]{\fboxx{ (np_{} \bs s_{})/ np_{} } \longrightarrow  (np_{} \bs s_{})/  \Diamond  \Box np_{} }{
 \infer[\bs ]{\fboxx{ np_{} \bs s_{} } \longrightarrow  np_{} \bs s_{} }{
 \infer{\fboxx{np_{}} \longrightarrow np_{}}{} &  \infer{\fboxx{s_{}} \longrightarrow s_{}}{}} &  \infer[\triangledown^{-1}]{ \Diamond  \Box np_{} \vdash np_{}}{ \infer[\Box ]{\fboxx{ \Box np_{}} \vdash  \Box np_{}}{ \infer{\fboxx{np_{}} \longrightarrow np_{}}{}}}} &  \infer[\slash ]{\fboxx{ (np_{} \bs s_{})/  \Diamond  \Box np_{} } \longrightarrow  (np_{} \bs s_{})/  \Diamond  \Box np_{} }{
 \infer[\bs ]{\fboxx{ np_{} \bs s_{} } \longrightarrow  np_{} \bs s_{} }{
 \infer{\fboxx{np_{}} \longrightarrow np_{}}{} &  \infer{\fboxx{s_{}} \longrightarrow s_{}}{}} &  \infer[\Diamond ]{ \Diamond  \Box np_{} \vdash \fboxx{ \Diamond  \Box np_{}}}{ \infer[\Box ]{\fboxx{ \Box np_{}} \vdash  \Box np_{}}{ \infer{\fboxx{np_{}} \longrightarrow np_{}}{}}}}}} &  \infer[\overline{\sigma}_\diamond]{ (gp_{}/ np_{}) \otimes (gp_{} \bs gp_{})  \vdash  gp_{}/  \Diamond  \Box np_{} }{
 \infer[\triangleright]{ (gp_{}/ np_{}) \otimes  \Diamond  \Box np_{}  \longrightarrow  gp_{}/ (gp_{} \bs gp_{}) }{
 \infer[\triangleleft^{-1}]{ ((gp_{}/ np_{}) \otimes  \Diamond  \Box np_{}) \otimes (gp_{} \bs gp_{})  \longrightarrow gp_{}}{
 \infer[\bs ]{\fboxx{ gp_{} \bs gp_{} } \longrightarrow  ((gp_{}/ np_{}) \otimes  \Diamond  \Box np_{}) \bs gp_{} }{
 \infer[\triangleright^{-1}]{ (gp_{}/ np_{}) \otimes  \Diamond  \Box np_{}  \longrightarrow gp_{}}{
 \infer[\slash ]{\fboxx{ gp_{}/ np_{} } \longrightarrow  gp_{}/  \Diamond  \Box np_{} }{
 \infer{\fboxx{gp_{}} \longrightarrow gp_{}}{} &  \infer[\triangledown^{-1}]{ \Diamond  \Box np_{} \vdash np_{}}{ \infer[\Box ]{\fboxx{ \Box np_{}} \vdash  \Box np_{}}{ \infer{\fboxx{np_{}} \longrightarrow np_{}}{}}}}} &  \infer{\fboxx{gp_{}} \longrightarrow gp_{}}{}}}}}}}}}}}}}}
}
\caption{``papers that reviewers rejected \textvisiblespace{} without reading \textvisiblespace{} carefully''}
\label{allrules}
\end{center}

\end{sidewaysfigure}

\begin{sidewaysfigure}
\begin{center}
\scalebox{.58}{\addtolength{\inferLineSkip}{3pt}
\infer=[]{n_{0}\otimes(\fboxx{ (n_{1} \bs n_{2})/ (s_{3}/  \Diamond  \Box np_{4}) }\otimes(np_{5} \otimes (((np_{6} \bs s_{7})/ np_{8}) \otimes  \Diamond (( \Box (((np_{9} \bs s_{10})/  \Diamond  \Box np_{11}) \bs ((np_{12} \bs s_{13})/  \Diamond  \Box np_{14}))/ (gp_{15}/  \Diamond  \Box np_{16})) \otimes ((gp_{17}/ np_{18}) \otimes (gp_{19} \bs gp_{20}))))))\longrightarrow n_{21}}{
 \infer[\slash ]{\fboxx{ (n_{1} \bs n_{2})/ (s_{3}/  \Diamond  \Box np_{4}) } \longrightarrow  (n_{0} \bs n_{21})/ (np_{5} \otimes (((np_{6} \bs s_{7})/ np_{8}) \otimes  \Diamond (( \Box (((np_{9} \bs s_{10})/  \Diamond  \Box np_{11}) \bs ((np_{12} \bs s_{13})/  \Diamond  \Box np_{14}))/ (gp_{15}/  \Diamond  \Box np_{16})) \otimes ((gp_{17}/ np_{18}) \otimes (gp_{19} \bs gp_{20}))))) }{
 \infer[\bs ]{\fboxx{ n_{1} \bs n_{2} } \longrightarrow  n_{0} \bs n_{21} }{
 \infer{\fboxx{n_{0}} \longrightarrow n_{1}}{} &  \infer{\fboxx{n_{2}} \longrightarrow n_{21}}{}} &  \infer[\overline{\alpha}_{\diamond}]{ np_{5} \otimes (((np_{6} \bs s_{7})/ np_{8}) \otimes  \Diamond (( \Box (((np_{9} \bs s_{10})/  \Diamond  \Box np_{11}) \bs ((np_{12} \bs s_{13})/  \Diamond  \Box np_{14}))/ (gp_{15}/  \Diamond  \Box np_{16})) \otimes ((gp_{17}/ np_{18}) \otimes (gp_{19} \bs gp_{20}))))  \longrightarrow  s_{3}/  \Diamond  \Box np_{4} }{
 \infer[\slash ]{\fboxx{  \Box (((np_{9} \bs s_{10})/  \Diamond  \Box np_{11}) \bs ((np_{12} \bs s_{13})/  \Diamond  \Box np_{14}))/ (gp_{15}/  \Diamond  \Box np_{16}) } \longrightarrow   \Box (((np_{6} \bs s_{7})/ np_{8}) \bs ((np_{5} \bs s_{3})/  \Diamond  \Box np_{4}))/ ((gp_{17}/ np_{18}) \otimes (gp_{19} \bs gp_{20})) }{
 \infer[\Box ]{\fboxx{ \Box (((np_{9} \bs s_{10})/  \Diamond  \Box np_{11}) \bs ((np_{12} \bs s_{13})/  \Diamond  \Box np_{14}))} \longrightarrow  \Box (((np_{6} \bs s_{7})/ np_{8}) \bs ((np_{5} \bs s_{3})/  \Diamond  \Box np_{4}))}{ \infer[\bs ]{\fboxx{ ((np_{9} \bs s_{10})/  \Diamond  \Box np_{11}) \bs ((np_{12} \bs s_{13})/  \Diamond  \Box np_{14}) } \longrightarrow  ((np_{6} \bs s_{7})/ np_{8}) \bs ((np_{5} \bs s_{3})/  \Diamond  \Box np_{4}) }{
 \infer[\slash ]{\fboxx{ (np_{6} \bs s_{7})/ np_{8} } \longrightarrow  (np_{9} \bs s_{10})/  \Diamond  \Box np_{11} }{
 \infer[\bs ]{\fboxx{ np_{6} \bs s_{7} } \longrightarrow  np_{9} \bs s_{10} }{
 \infer{\fboxx{np_{9}} \longrightarrow np_{6}}{} &  \infer{\fboxx{s_{7}} \longrightarrow s_{10}}{}} &  \infer[\Box ]{\fboxx{ \Box np_{11}} \longrightarrow  \Box np_{8}}{ \infer{\fboxx{np_{11}} \longrightarrow np_{8}}{}}} &  \infer[\slash ]{\fboxx{ (np_{12} \bs s_{13})/  \Diamond  \Box np_{14} } \longrightarrow  (np_{5} \bs s_{3})/  \Diamond  \Box np_{4} }{
 \infer[\bs ]{\fboxx{ np_{12} \bs s_{13} } \longrightarrow  np_{5} \bs s_{3} }{
 \infer{\fboxx{np_{5}} \longrightarrow np_{12}}{} &  \infer{\fboxx{s_{13}} \longrightarrow s_{3}}{}} &  \infer[\Diamond ]{ \Diamond  \Box np_{4} \longrightarrow \fboxx{ \Diamond  \Box np_{14}}}{ \infer[\Box ]{\fboxx{ \Box np_{4}} \longrightarrow  \Box np_{14}}{ \infer{\fboxx{np_{4}} \longrightarrow np_{14}}{}}}}}} &  \infer[\overline{\sigma}_{\diamond}]{ (gp_{17}/ np_{18}) \otimes (gp_{19} \bs gp_{20})  \longrightarrow  gp_{15}/  \Diamond  \Box np_{16} }{
 \infer[\bs ]{\fboxx{ gp_{19} \bs gp_{20} } \longrightarrow  ((gp_{17}/ np_{18}) \otimes  \Diamond  \Box np_{16}) \bs gp_{15} }{
 \infer[\slash ]{\fboxx{ gp_{17}/ np_{18} } \longrightarrow  gp_{19}/  \Diamond  \Box np_{16} }{
 \infer{\fboxx{gp_{17}} \longrightarrow gp_{19}}{} &  \infer[\Box ]{\fboxx{ \Box np_{16}} \longrightarrow  \Box np_{18}}{ \infer{\fboxx{np_{16}} \longrightarrow np_{18}}{}}} &  \infer{\fboxx{gp_{20}} \longrightarrow gp_{15}}{}}}}}}}
 }
\caption{Example (\ref{data2}d), non-invertible rules, indexed atomic formula occurrences.}
\label{noninvertiblerules} 
\end{center}
\end{sidewaysfigure}




==> Sections/BSyntaxDiagrams.tex <==
\begin{figure}[h]
\begin{center}
	    \tikzdiagramsmall{0.65}{infoflow_parasitic_gap_simple1}
	    \vspace{-3em}
\end{center}
\caption{Paper that Bob rejected immediately.}
\label{fig:infoflow_parasitic_gap}
\end{figure}

\begin{figure}[h]
\begin{center}
	    \tikzdiagramsmall{0.65}{infoflow_parasitic_gap_simple2}
\end{center}
\caption{``Bob left without closing the window." We indicate the island (effectuated by the modal decoration in the type for `without') with the dashed lines.}
\label{fig:infoflow_parasitic_gap}
\end{figure}

\begin{figure}[h]
\begin{center}
	    \tikzdiagramsmall{0.65}{infoflow_parasitic_gap_simple3}
\end{center}
\caption{Failing to derive ``window that Bob left without closing." The hypothetical noun phrase is situated within an island, and can't escape out to form the sentence missing a noun phrase that is required by the relative pronoun.}
\label{fig:infoflow_parasitic_gap_fail}
\end{figure}


\begin{sidewaysfigure}[h]
\begin{center}
	    \tikzdiagramsmall{0.65}{infoflow_parasitic_gap}
	    \vspace{-4em}
\end{center}
\caption{Information flow for the double parasitic gap.}
\label{fig:infoflow_parasitic_gap}
\end{sidewaysfigure}

\begin{sidewaysfigure}
    \begin{center}
        \tikzdiagramsmall{0.6}{infoflow_parasitic_subject_en}     
    \end{center}
    \caption{Information flow for the double parasitic gap in subject position.}
    \label{fig:infoflow_parasitic_gap_subject}
\end{sidewaysfigure}



==> Sections/StringDiagrams.tex <==
\section{Picturing Lambek Processes}

To make the given proofs more accessible, we provide string diagrams in the style of \cite{wijnholds2017coherent} for proofs of the system \textbf{NL}$_{\fdia}$.


\begin{sidewaysfigure}
    \begin{center}
	    \tikzdiagramsmall{0.6}{infoflow_parasitic_gap}
    \end{center}
    \caption{Information flow for the double parasitic gap.}
    \label{fig:infoflow_parasitic_gap}
\end{sidewaysfigure}

\begin{sidewaysfigure}
    \begin{center}
	    \tikzfig{infoflow_parasitic_gap_ccc}
    \end{center}
    \caption{CCC Information flow for the double parasitic gap.}
    \label{fig:infoflow_parasitic_gap_ccc}
\end{sidewaysfigure}

\begin{sidewaysfigure}
    \begin{center}
        \tikzdiagramsmall{0.6}{infoflow_parasitic_subject_en}     
    \end{center}
    \caption{Information flow for the double parasitic gap in subject position.}
    \label{fig:infoflow_parasitic_gap_subject}
\end{sidewaysfigure}
